The Chronicles of Radio Frequency Fingerprinting

Radio Frequency Fingerprinting (RFF) has evolved from an early idea for radar emitter identification into a broad research field for wireless device identification and spectrum monitoring for security. Rather than presenting a conventional literature survey, this work provides a critical historical analysis of RFF organized around the field's major conceptual paradigm shifts from 1993 to 2026. We discuss the evolution of RFF across its fundamental methodological phases, beginning with early transient-based approaches, in which transmitter turn-on behavior, unintentional modulation, and hardware nonlinearities were treated as the primary fingerprint sources. We then examine the transition to digital communications, during which attention shifted to steady-state impairments and to engineered features extracted from signals. Next, we discuss the Machine Learning period, which standardized the RFF workflow around feature extraction, dimensionality reduction, and supervised classification, followed by the Deep Learning period, in which representation learning from raw IQ samples significantly improved performance and expanded the application space. Beyond a chronological list of methods and best practices, this paper critically examines the changing assumptions and persistent limitations that have driven these transitions. We highlight the central challenges that continue to shape the field, including channel dependence, receiver sensitivity, limited dataset realism, poor cross-domain generalization, open-set recognition, and adversarial robustness. By organizing more than three decades of work into a coherent narrative, this paper clarifies the evolution of RFF, identifies persistent limitations, and outlines the key research directions required to move the field toward dependable real-world adoption.

==> acronyms.tex <==
\acrodef{AGC}{Automatic Gain Control}
\acrodef{AI}{Artificial Intelligence}
\acrodef{AML}{Adversarial Machine Learning}
\acrodef{ANN}{Artificial Neural Network}
\acrodef{AUC}{Area Under the Curve}
\acrodef{ADS-B}{Automatic Dependent Surveillance-Broadcast}
\acrodef{BER}{Bit Error Rate}
\acrodef{BPSK}{Binary Phase-Shift Keying}
\acrodef{CFNN}{Complex Fourier Neural Network}
\acrodef{CFO}{Carrier Frequency Offset}
\acrodef{CNN}{Convolutional Neural Network}
\acrodef{CSI}{Channel State Information}
\acrodef{CVCNN}{Complex-Valued Convolutional Neural Network}
\acrodef{CVNN}{Complex-Valued Neural Network}
\acrodef{DF}{Device Fingerprint}
\acrodef{DL}{Deep Learning}
\acrodef{DSP}{Digital Signal Processing}
\acrodef{FCNN}{Fully Connected Neural Network}
\acrodef{FGSM}{Fast Gradient Signed Method}
\acrodef{FPGA}{Field-Programmable Gate Array}
\acrodef{FPR}{False Positive Rate}
\acrodef{GAN}{Generative Adversarial Network}
\acrodef{GCS}{Ground Control Station}
\acrodef{Grad-CAM}{Gradient-weighted Class Activation Mapping}
\acrodef{GPP}{General-Purpose Processor}
\acrodef{GRU}{Gated Recurrent Unit}
\acrodef{HPC}{High-Performance Computing}
\acrodef{IoT}{Internet of Things}
\acrodef{IoU}{Intersection over Union}
\acrodef{IQ}{In-Phase and Quadrature}
\acrodef{ISAC}{Integrated Sensing and Communications}
\acrodef{KNN}{K-Nearest Neighbors}
\acrodef{LIME}{Local Interpretable Model-agnostic Explanations}
\acrodef{LS}{Least-Squares}
\acrodef{LoRa}{Long Range}
\acrodef{LSTM}{Long Short-Term Memory}
\acrodef{LTE}{Long Term Evolution}
\acrodef{MAC}{Media Access Control}
\acrodef{MCA}{Multi-Class AdaBoost}
\acrodef{ML}{Machine Learning}
\acrodef{MLP}{Multi-Layer Perceptron}
\acrodef{MMSE}{Minimum Mean-Square Error}
\acrodef{MSE}{Mean-Square Error}
\acrodef{NN}{Neural Network}
\acrodef{OFDM}{Orthogonal Frequency-Division Multiplexing}
\acrodef{PCA}{Principal Component Analysis}
\acrodef{PHY}{Physical}
\acrodef{PLA}{Physical Layer Authentication}
\acrodef{PLC}{Power Line Communication}
\acrodef{PLS}{Physical Layer Security}
\acrodef{PNN}{Probabilistic Neural Network}
\acrodef{PSK}{Phase-Shift Keying}
\acrodef{QPSK}{Quadrature Phase-Shift Keying}
\acrodef{ReLU}{Rectified Linear Unit}
\acrodef{RF}{Radio Frequency}
\acrodef{RFF}{Radio Frequency Fingerprinting}
\acrodef{RFFI}{Radio Frequency Fingerprint Identification}
\acrodef{RFID}{Radio Frequency Identification}
\acrodef{RFMLS}{Radio Frequency Machine Learning System}
\acrodef{RGB}{Red-Green-Blue}
\acrodef{RNN}{Recurrent Neural Network}
\acrodef{ROC}{Receiver-Operating Characteristic}
\acrodef{RRC}{Root Raised Cosine}
\acrodef{RSSI}{Received Signal Strength Indicator}
\acrodef{SDR}{Software-Defined Radio}
\acrodef{SEI}{Specific Emitter Identification}
\acrodef{SHAP}{SHapley Additive exPlanations}
\acrodef{SNR}{Signal-to-Noise Ratio}
\acrodef{SSB}{Synchronization Signal Blocks}
\acrodef{SSL}{Self-Supervised Learning}
\acrodef{SVM}{Support Vector Machine}
\acrodef{TL}{Transfer Learning}
\acrodef{UAV}{Unmanned Aerial Vehicle}
\acrodef{UHF}{Ultra High Frequency}
\acrodef{UMOP}{Unintentional Modulation on Pulse}
\acrodef{USRP}{Universal Software Radio Peripheral}
\acrodef{VHF}{Very High Frequency}
\acrodef{XAI}{eXplainable AI}
